Graph versioning for evolving urban data

The continuous evolution of cities poses significant challenges in terms of managing and understanding their complex dynamics. With the increasing demand for transparency and the growing availability of open urban data, it has become important to ensure the reproducibility of scientific research and computations in urban planning. To understand past decisions and other possible scenarios, we require solutions that go beyond the management of urban knowledge graphs. In this work, we explore existing solutions and their limits and explain the need and possible approaches for querying across multiple graph versions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=project

PDF = $(PACKAGE).pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

all:  ${PDF}

%.pdf:
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex -synctex=1 -interaction=nonstopmode -file-line-error $<; done

%.cls:   %.ins %.dtx
	pdflatex $<

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	./**/*.log ./**/*.aux \
	./**/*.cfg ./**/*.glo ./**/*.idx ./**/*.toc \
	./**/*.ilg ./**/*.ind ./**/*.out ./**/*.lof \
	./**/*.lot ./**/*.bbl ./**/*.blg ./**/*.gls ./**/*.cut ./**/*.hd \
	./**/*.dvi ./**/*.ps ./**/*.thm ./**/*.tgz ./**/*.zip ./**/*.rpi

clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE).synctex.gz

distclean: clean
	$(RM)  *.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

.PHONY: all docclean clean distclean archive zip

